Swazure: Swarm Measurement of Pose for Flying Light Specks

One may construct a 3D multimedia display using miniature drones configured with light sources, Flying Light Specks (FLSs). Swarms of FLSs localize to illuminate complex 3D shapes and animated sequences consistent with the coordinates of points in a point cloud. This requires FLSs to accurately measure their pose relative to one another using sensors such as cameras. Such sensors have a sweet range in which they provide the highest accuracy. A challenge is how an FLS tracks another FLS outside its sensor's sweet range, dictated by the point cloud data. We address this challenge by proposing a novel technique called Swazure that solves the missing sensor data using cooperation among FLSs. It implements physical data independence by abstracting the physical characteristics of the sensors, making point cloud data independent of the sensor hardware. The size of an FLS relative to the minimum distance between points of a point cloud is an important parameter. With medium-sized FLSs, Swazure is able to position 100% of the FLS's neighbors. Larger FLS sizes may result in potential obstructions that prevent Swazure from quantifying relative pose. We present two heuristics, Move Obstructing and Move Source, to address this limitation. Our experimental results show the superiority of the Move Obstructing heuristic which resolves approximately 30% of obstructions in the worst case scenario.

==> abstOLD.tex <==
Consider a sensor with a minimum range (say 6 centimeters) and an application that must quantify distances smaller than this range (say 7 millimeters).
Swarm measurement, Swazure, enables the application by requiring devices using these sensors to cooperate and share their relative pose information with one another.
We illustrate Swazure with a swarm of drones that illuminate 3D multimedia shapes.
Each drone is configured with a Raspberry camera and an ArUco marker.
This setup enables a drone to quantify distances with millimeter accuracy as long as the range is between 6 to 8 centimeters, i.e., the {\em sweet} range.
It is not able to measure distances shorter than 5 centimeters.  
Swazure enables the drones to quantify their average distance of 7 millimeters with a high accuracy.
%An assumption is that the overall size of the multimedia shape exceeds the sweet range of the sensor.

==> concOLD.tex <==
Swazure enables an FLS to compute its relative pose to a neighboring FLS with a high accuracy when the neighbor is too close, preventing its sensor from quantify the pose.
It abstracts the range of a sensor into a blind, sweet, and decaying range.
It requires the FLSs to cooperate and share information about their sweet neighbors.  
In this paper, we illustrated Swazure using FLSs configured with inexpensive Raspberry camera and an ArUco marker~\cite{swarical2024} to illuminate point clouds consisting of hundreds and thousands of points (FLSs).
In general, Swazure may be used with any application that requires its devices to compute their relative pose at blind ranges of their sensors.
A key requirement is reliable communication between FLSs.
Another requirement is for every device to have a sweet neighbor.
When this requirement is violated, one may consider injecting additional devices that satisfy this requirement.
This is similar to Swarical injecting dark FLSs to localize a point cloud~\cite{swarical2024} or an availability technique using dark standby FLSs~\cite{reliability2024}.
We defer the details of Swazure's extensions to future work once we identify an application that violates our requirement.

==> oldMoveObstSource.tex <==
These techniques are highly effective in reducing both the average and maximum error in distance, $\alpha$, $\theta$, and $\phi$.
This is especially true with $\beta=0.5$ which incurs the highest error.
For example, with the Kangaroo and $\beta=0.5$, these techniques reduce the maximum percentage error in distance by more than 99\%, from 671\% down to 2.55\% with Move Obstructing and 5.21\% with Move Source.





While these techniques improve the {\em maximum} error in $\phi$, their impact is not as significant as that with $\theta$ and $\alpha$.
For example, with the Dragon and $\beta=0.5$, Move Obstructing reduces the maximum $\theta$ error from 120$^{\circ}$ to 0.84$^{\circ}$.
However, it improves the maximum $\phi$ error from 179.91$^{\circ}$ to only 43$^{\circ}$.
This observation applies to all shapes and $\beta$ values.
This is because the direction of the estimated and ground truth vectors impacts the $\phi$ error. The more they are aligned with the z-axis, the larger the $\phi$ error may become because the projected vectors on the x-y plane have a larger angle between them than the original vectors. 
In our experiments with Move Obstructing, all of the ground truth poses between FLS pairs with the maximum $\phi$ error are approximately directed towards the z-axis.
This explanation also describes why the use of Move Obstructing and Move Source may not enhance (reduce) the maximum $\phi$ with the Race Car and the Skateboard.  With both shapes, the maximum $\phi$ error increases for certain $\beta$ values.  

%The $\phi$ angle from the spherical coordinates does not necessarily indicate whether a technique improves the estimation or not. It 
%has two main caveats.
%To illustrate, consider the estimated poses $\relpose{1}{n}^1=(2.094e-3, -6.606e-4, 3.595)$ and $\relpose{1}{n}^2=(2.057e-3, 5.120e-3, 3.585)$ for a pair of FLS using the Shortest Path and Move Obstructing techniques respectively. The ground truth pose for this pair is $\relposegt{1}{n}~=(-7.072e-4, -2.529e-3, 3.547)$. The first caveat is that while the $\alpha$ angle for both techniques is less than one degree (0.05° and 0.13°), the error in their $\phi$ is 88.11° and 173.73°, respectively, which is dramatically a larger value. The second caveat is that despite the $\alpha$ angle being smaller for the Move Obstructing technique, its corresponding $\phi$ error is higher than that of the Shortest Path technique. This indicates that $\phi$ error may increase even when a technique improves accuracy. This is because $\relposegt{1}{n}$ is almost aligned with the z-axis, and slight variation in the x or y components of the $\relpose{1}{n}$ can cause significant changes in the $\phi$ angle.


\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{figs/dragonDistErrHopsLengthHist.jpg}
    \caption{Histogram of percentage error in distance, Dragon $\beta=0.5$.}
    \label{fig:dragon-dist-err}
\end{figure}

These techniques are effective because they either reduce the number of hops in a path or reduce the length of a path by replacing one or more decaying hops of a path with sweet hops.
For example, with the Kangroo and $\beta=0.5$, Move Obstructing reduces the average number of hops by the Shortest-Length from 2.27 to 2.06.
Moreover, it reduces the average length of the path computed by Shortest-Length from 14.61 to 12.81.

Move Obstructing is superior to Move Source because it minimizes the distance travelled by an FLS.
Its reduction is orders of magnitude lower.  
For example, with the Kangroo and $\beta=0.5$, the average distance moved by the blocking FLS is 1.6 display cells with Move Obstructing.
With Move Source, this average increases to 215 display cells. 
It is important to note that with $\beta$ values lower than X, these techniques are not used with all the shapes.



\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{figs/avgDistMovedKangarooHopBeta.jpg}
    \caption{Average distance moved by source FLS and average distance moved by obstructing FLSs for Kangaroo.}
    \label{fig:dist-moved}
\end{figure}


\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{figs/percentageSuccessHopBeta.jpg}
    \caption{Percentage success of Move Obstructing and Move Source techniques for Kangaroo.}
    \label{fig:success-rate}
\end{figure}
